Classifier-Free Guidance is a Predictor-Corrector

We investigate the theoretical foundations of classifier-free guidance (CFG). CFG is the dominant method of conditional sampling for text-to-image diffusion models, yet unlike other aspects of diffusion, it remains on shaky theoretical footing. In this paper, we disprove common misconceptions, by showing that CFG interacts differently with DDPM (Ho et al., 2020) and DDIM (Song et al., 2021), and neither sampler with CFG generates the gamma-powered distribution $p(x|c)^\gamma p(x)^{1-\gamma}$. Then, we clarify the behavior of CFG by showing that it is a kind of predictor-corrector method (Song et al., 2020) that alternates between denoising and sharpening, which we call predictor-corrector guidance (PCG). We prove that in the SDE limit, CFG is actually equivalent to combining a DDIM predictor for the conditional distribution together with a Langevin dynamics corrector for a gamma-powered distribution (with a carefully chosen gamma). Our work thus provides a lens to theoretically understand CFG by embedding it in a broader design space of principled sampling methods.

==> cfg_as_pcg_old.tex <==

Claims:
\begin{enumerate}
  \item DDPM-CFG$(\gamma)$ is equivalent to DDIM-PCG($2\gamma-1$)
    \item (TBD) PCG of some kind is similar to CFG++, and to Karras
    \item (TBD?): DDIM-PCG can be thought of as ``approximately'' sampling $p_{0, \gamma}$.
\end{enumerate}



Notice that this is actually the same as DDPM-CFG with a different gamma!
\begin{align}
\boxed{
\textsf{DDIM-PCG}_t(x, \gamma)
\equiv
\textsf{DDPM-CFG}_t(x, \half + \frac{\gamma}{2})
}
\end{align}
Proof in \ref{app:cfg_pcg_proof}.

Insights about CFG:
This means that DDPM-CFG can be thought of as alternating between a single step of DDIM denoising and a single step of LD on $p_{t, \gamma}(x|c)$. The LD step moves toward its steady-state $p_{t, \gamma}(x|c)$, the sharpened conditional noisy distribution, but only by a single step (so it only moves toward the SS but does not reach it). 

==> cfg_structure.tex <==
\section{Structural Characterization of CFG}
Having appreciated the subtlety of CFG, we can now state our main structural
characterization.

As a warm-up, suppose we actually wanted to sample from the
distribution $p_\gamma$ defined in Equation~\eqref{eqn:intro-pgamma}.
How would we do this, given access to standard score models 
for $p(x)$ and $p(x \mid c)$? 
A natural strategy is to run Langevin dynamics (LD) w.r.t. $p_\gamma$.
This is possible in theory because 
we can compute the score of $p_\gamma$ from the known scores of $p(x)$
and $p(x\mid c)$:
\begin{align}
\grad_x \log p_\gamma(x \mid c) = (1-\gamma) \grad_x \log p(x)
+ \gamma \grad_x \log p(x \mid c)
\end{align}
However this won't work in practice, due to the well-known issue
that vanilla Langevin dynamics has impractically slow mixing times for
many distributions of interest, e.g. images \citep{song2019generative}.
The usual remedy for this is to use some kind of annealing...

\pnote{todo.}

\pnote{Todo: DDPM-CFG = DDIM + LD$_\gamma$ claim.}

==> scratch.tex <==

\section{Scratch}


\begin{figure}
    \centering
    \includegraphics[width=1.0\textwidth]{fig/pcg_hero.png}
    \caption{}
    \label{fig:hero}
\end{figure}

Suppose we want to sample from p-gamma, given lots of compute, and score-function.
What would we do? 
First choice: LD on p-gamma, since we have scores.
Lessons from diffusion: slow-mixing time / not working when deadzones.
(maybe SMLD)
Natural choice: predictor-corrector.
We have a "crude predictor" (denoiser), and a "correct" corrector (LD on the score).
This method was known, but underappreciated -- usually applied where P and C are w.r.t. the same distribution.
Let's try this...
Apriori, seems unrelated to CFG.

\begin{itemize}
    \item CFG turns out to be equivalent (in the SDE limit) to the algo described as DDIM-PCG.
    (BUT: slightly different gamma!)
    \item Thus, CFG can be formally interprepreted as a P-C algorithm
    (denoising and sharpening).
    \item This naturally opens a broader design space, which we call PCG family of samplers.
    (in fact, connected to Karras and CFG++).
    \item Experimentally, PCG methods produce good samples (given compute).
    \item Lesson from experiments: Sometimes possible to get good samples WITHOUT CFG.
    (So, benefits of CFG may be just the "implicit corrector").
\end{itemize}


\begin{enumerate}
    \item Theorem: CFG does not generate the $\gamma$-powered distribution.
    \item Theorem: DDIM-CFG does not generate equivalent distribution as DDPM-CFG.
    \item DDPM-CFG$(\gamma)$ is equivalent to DDIM-PCG($2\gamma-1$)
    \item (maybe?): DDIM-PCG can be thought of as ``approximately'' sampling $p_{0, \gamma}$.
    \item Experimentally: LD helps DDPM a lot.
    Conditional sampling (unsharpened) can produce
    high-quality samples, with LD steps. 
\end{enumerate}

\subsection{Claims}
\begin{enumerate}
    \item Discussion: Why is the heuristic derivation of CFG problematic? (No clear fwd process, not a diffusion, etc).
    \item Theorem: CFG does not generate the $\gamma$-powered distribution.
    \item Theorem: DDIM-CFG does not generate equivalent distribution as DDPM-CFG. DDIM over-sharpens a lot. BUT they can be similar (1g gaussian).
\end{enumerate}

Sharpening the conditional distribution focuses more prototypical examples of a given condition: for example in text-to-image diffusion with the prompt "broccoli" the sharpened conditional would produce images with higher alignment with the prompt. The training distribution conditioned on text "broccoli" may in fact be more diverse than we wish, containing many examples with only a weak adherence to the prompt, while we might wish to generate only the "best" images (highest image quality with strongest connection to the prompt).


The DDPM discrete update \citep{ho2020denoising} is:
\begin{align}
    x_{t+\dt} &= \sqrt{1 - \beta_{t+\dt}} x_{t} + \beta_{t+\dt} \xi, \quad \xi \sim \mathcal{N}(0,1) \label{eq:ddpm_discrete} \\
    \implies x_t &= F_t(x_0, \epsilon) := \sqrt{\bar \alpha_{t}} x_0 + (1-\bar \alpha_{t}) \xi, \quad \bar \alpha_t = \prod_{j=0}^{t/\dt} (1-\beta_{j\dt}) \\
    \implies p_t(x_t) &= F_t \sharp (p_0(x_0), p_\epsilon(\epsilon)), \quad p_\epsilon \sim \cN(0,1)
\end{align}

\subsection{SDE Limit of PCG}
At timestep $t$:
\begin{enumerate}
    \item Predictor: Take one DDIM/DDPM step for $p_t(x|c)$.
    That is, using score $ \nabla \log p_t(x | c)$.
    
    \item Corrector: Take Langevin dynamics step(s) with target
    distribution $p_{t, \gamma}$.
    That is, run the below SDE for any amount of time $s$.
    Note that $s$ starts at $0$ and increases, and $s$ is unrelated to $t$.
\begin{align}
    dx &= \half \nabla_x \log p_{t, \gamma}(x) ds + dw'  \\
    &= \half 
     (1-\gamma)\nabla \log p_t(x) ds + \half \gamma \nabla \log p_t(x | c)  ds +  dw'
\end{align}
where $w'$ is a Brownian motion w.r.t. time $s$ (NOT w.r.t. time $t$), which is independent of $dw$ in the DDPM formula above.
\end{enumerate}


We are free to chose how $s$ should be related to $t$.
Let us for simplicity pick $ds = -C \beta_t dt$, which changes $dw'$ to $\sqrt{C\beta_t}d\bar{w}'$, . This ensures that at $C=1$, the scale of the Langevin noise term $\sqrt{C\beta_t}d\bar{w}'$ matches that of DDPM $\beta_t d\bar{w}$, although the two are independent.
The factor $C$ is essentially ``how long should we run the LD, at each diffusion step.''
With this choice, the Langevin SDE becomes:
\begin{align}
dx &=
- \half C \beta_t (1-\gamma)\nabla \log p_t(x) dt
- \half C \beta_t \gamma \nabla \log p_t(x | c)  dt 
+  \sqrt{C\beta_t} d\bar{w}'
\end{align}
where $d\bar{w}'$ is the time-reversal of $dw'$.
\\\\
Interpretation:
\\
Predictor-Corrector: The predictor step is standard diffusion denoising, while the corrector strengthens the conditioning via LD on a sharpened conditional distribution [or possibly GD on the score of the $p(x|c)$ which is more like CFG++, or any other algorithm that somehow strengthens the conditioning.]
\\\\
- In the limit of zero LD steps, PCG is a standard diffusion denoiser.
\\
- In the limit of infinite LD steps, PCG converges exactly to the LD SS (i.e. the sharpened conditional distribution).
\\
- In between, PCG balances between denosing and sharpening.
\\
- For one or more LD steps on $p_t(x|c)$, PCG is just PC. 
\\
PCG is similar to CFG++ (see Appendix \ref{app:cfg_pp_as_pcg})
\\
- For a single step of LD on $p_{t,\gamma}(x|c)$, PCG (for particular choices) exactly reproduces CFG (and relates strongly to CFG++).


- Karras CFG can be written as PCG with LD on $p_{t, \gamma}$ except with a "worse" model instead of an unconditional model.

